Structured Multi-Label Biomedical Text Tagging via Attentive Neural Tree Decoding

We propose a model for tagging unstructured texts with an arbitrary number of terms drawn from a tree-structured vocabulary (i.e., an ontology). We treat this as a special case of sequence-to-sequence learning in which the decoder begins at the root node of an ontological tree and recursively elects to expand child nodes as a function of the input text, the current node, and the latent decoder state. In our experiments the proposed method outperforms state-of-the-art approaches on the important task of automatically assigning MeSH terms to biomedical abstracts.

==> relatedworks.tex <==
% bcw 1/9: for short papers, typically best to merge related work with the intro
\section{Related Work}

\label{section:related-work}

%We will overview two different threads of work that are relevant to this paper: 1) research on automated biomedical text annotation and 2) then approaches to structured multilabel classification

\subsection{Sequence-to-Sequence Learning}
\label{section:related-work:seq2seq}

Our model follows the general paradigm of \emph{seq2seq} learning, first popularized by 
\newcite{sutskever2014sequence}. These are architectures for mapping from input to output sequences, e.g., from a source to a target language, in the case of translation. Seq2seq models must specify an encoder $\mathtt{enc}$ and a decoder $\mathtt{dec}$, parameterized by $\theta_{\mathtt{enc}}$ and $\theta_{\mathtt{dec}}$, respectively. An input sequence $x_i=\{x_i^1, x_i^2, ... x_i^n\}$ is first compressed into a latent representation $h_i=\mathtt{enc}(x_i|\theta_{\mathtt{enc}})$. This is then consumed by the decoder, which is tasked with mapping latent representations to target sequences: $y_i=\{y_i^1, y_i^2, ... y_i^m\}=\mathtt{dec}(h_i|\theta_{\mathtt{dec}})$. 


One issue in this simple seq2seq formulation is that all salient information necessary for decoding must be packed into $h_i$. This may prove difficult and hence hinder model performance. To mitigate this, \newcite{bahdanau2014neural} proposed \emph{attention}, a mechanism for allowing the decoder to focus on the most relevant bits of the input at a given step in the decoding process. In particular, at each step in the decoding process, the decoder model induces a distribution over inputs such that tokens relevant for the current prediction are emphasized.\footnote{This may be viewed as a context-specific, soft alignment between the output being generated and the input sequence.} 

Most instances of seq2seq architectures have been proposed for applications that assume ``structure-free'' decoding, i.e., where the target is an unconstrained sequence of symbols. Recently, however, there has been increased interest in decoders that effectively output structures \cite{duvsek2016sequence,roee-acl017,dong2016language,xiao2016sequence,alvarez2016tree,tai2015improved}. A common strategy here is to treat the target output sequence as string that specifies a tree structure. For example, \newcite{roee-acl017} proposed a neural translation model that maps source languages directly into linearized English constituency trees (which codify syntactic structure). Similarly, in the domain of semantic parsing, \newcite{dong2016language} proposed mapping unstructured input queries to strings specifying logical forms. These works can be seen as trying to \emph{generate} structure during decoding, whereas in our case we are \emph{constrained} by it. Thus, rather than generating nodes, we select them. 


% (much of this work has been focused on the application of translation)
%of this work has been focussed on the domain of translation, e.g.,

%Improvements have been reported in the seq-to-seq deep models using attention \cite{bahdanau2014neural, paulus2017deep}.  The proposed approach in this work of decoding into a tree mildly resembles structure-aware seq-to-seq learning \cite{liu2017table}.

Perhaps the work most relevant to the present effort that we have found is a preliminary (unpublished) description of a system that attempts to perform concept-linking from free-texts to ontologies \cite{fuconcept}. In particular, this model aims to map spans of text from patient notes to standardized concepts in the SNOWMED biomedical ontology. An attempt was made to use a seq2seq architecture that traversed the ontology graph structure, as we propose here; however the results were very poor as compared to simple baseline models. The problem considered by \cite{fuconcept} differs from the present effort in two fundamental ways: first, their task was easier than ours, in that model inputs were short spans of text, as opposed to lengthier abstracts to be annotated. This motivates our use of an attention mechanism, conditioned on the current stage of graph traversal. Second, they had orders of magnitude less labeled data than us, which likely explains their negative finding (as the author himself suggests). 

\subsection{Biomedical Text Annotation}
Biomedical natural language processing is a broad, active field \cite{zweigenbaum2007frontiers, demner2016aspiring}. Here we review the literature that deals with text annotation.  One early system that was used to extract clinical trial characteristics from free-texts is ExaCT \cite{Kiritchenko2010}, which is aimed at identifying and extracting data elements from free texts describing clinical trials necessary for evidence synthesis. ExaCT uses a mixture of statistical and rule based approaches. In \cite{neveol2007multiple}, they use heuristics, dictionary based mapping of text to mesh heading and learn nlp based rules that can be used to predict mesh terms. Tsuruoka \textit{et al.} \cite{Tsuruoka2005} presents a part-of-speech tagger which was specifically tuned for biomedical text. 
% Summerscales \cite{summerscales2011automatic} developed a similar system, which attempted to automatically calculate summary statistics reported in an abstract by first identifying treatment group and outcome mentions and then processing numerical quantities in the text with reference to these. 

BIOASQ\footnote{\url{http://bioasq.org/}} challenge runs a task for mesh annotation; \cite{liu2014fudan, tsoumakas2013large} performed well in that task in two different years.  More recently, Singh \emph{et al.} \cite{Singh:2017:NCA:3132847.3132989} proposed a neural candidate-selector architecture that starts from a high recall and low precision candidate set of mesh terms, followed by pruning to obtain precise annotation terms. The work is based on using a deep model that can learn joint distribution of terms with small amounts of annotated data. 

\subsection{Structured Multilabel Classification}
The task of mesh term prediction can be viewed as an instance of structured multilabel classification. A lot of work has been done in the area of general multilabel classification, e.g., \cite{elisseeff2002kernel, furnkranz2008multilabel, read2011classifier}. It is difficult to learn an accurate multilabel classifier that can predict in domains with large output space \cite{tsochantaridis2004support, tsoumakas2008effective}. One way to deal with such large label spaces is to use label space reduction methods \cite{bi2013efficient, chen2012feature, ji2009linear}. 

More relevant to the current work, multilabel classification for text has received a fair amount of attention in the past \cite{katakis2008multilabel, mccallum1999multi}. One way to approach multilabel classification is to posit a generative mixture model wherein documents are associated with a set of labels that are in turn ascribed a partial responsibility for generating the words describing a particular document \cite{mccallum1999multi}. 

%\subsection{Sequence-to-Sequence Learning}

